Weighted Maximum Likelihood for Controller Tuning

Recently, Model Predictive Contouring Control (MPCC) has arisen as the state-of-the-art approach for model-based agile flight. MPCC benefits from great flexibility in trading-off between progress maximization and path following at runtime without relying on globally optimized trajectories. However, finding the optimal set of tuning parameters for MPCC is challenging because (i) the full quadrotor dynamics are non-linear, (ii) the cost function is highly non-convex, and (iii) of the high dimensionality of the hyperparameter space. This paper leverages a probabilistic Policy Search method - Weighted Maximum Likelihood (WML)- to automatically learn the optimal objective for MPCC. WML is sample-efficient due to its closed-form solution for updating the learning parameters. Additionally, the data efficiency provided by the use of a model-based approach allows us to directly train in a high-fidelity simulator, which in turn makes our approach able to transfer zero-shot to the real world. We validate our approach in the real world, where we show that our method outperforms both the previous manually tuned controller and the state-of-the-art auto-tuning baseline reaching speeds of 75 km/h.

==> Figures/lap_time.tex <==
% This file was created with tikzplotlib v0.9.16.
\begin{tikzpicture}

\begin{axis}[
width=0.5\textwidth,
height=0.3\textwidth,
axis x line=top,
x grid style={white!69.0196078431373!black},
xmajorgrids,
xmin=0.5, xmax=5.5,
xtick pos=right,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabels={MPC, Marvin, Gabriel, MPCC,  \textbf{Ours} },
y grid style={white!69.0196078431373!black},
ylabel={Lap Time (\(\displaystyle s\))},
ymajorgrids,
ymin=4.5, ymax=6.5,
ytick pos=both,
ytick style={color=black},
ytick={4.5, 5, 5.5, 6, 6.5},
yticklabels={
  \(\displaystyle {4.50}\),
%   \(\displaystyle {4.75}\),
  \(\displaystyle {5.00}\),
%   \(\displaystyle {5.25}\),
  \(\displaystyle {5.50}\),
%   \(\displaystyle {5.75}\),
  \(\displaystyle {6.00}\),
%   \(\displaystyle {6.25}\),
  \(\displaystyle {6.50}\)
}
]
\addplot [black]
table {%
0.75 6.129
1.25 6.129
1.25 6.15
0.75 6.15
0.75 6.129
};
\addplot [black]
table {%
1 6.129
1 6.127
};
\addplot [black]
table {%
1 6.15
1 6.16
};
\addplot [black]
table {%
0.875 6.127
1.125 6.127
};
\addplot [black]
table {%
0.875 6.16
1.125 6.16
};
\addplot [black]
table {%
1.75 5.772
2.25 5.772
2.25 5.772
1.75 5.772
1.75 5.772
};
\addplot [black]
table {%
2 5.772
2 5.772
};
\addplot [black]
table {%
2 5.772
2 5.772
};
\addplot [black]
table {%
1.875 5.772
2.125 5.772
};
\addplot [black]
table {%
1.875 5.772
2.125 5.772
};
\addplot [black]
table {%
2.75 5.678
3.25 5.678
3.25 5.678
2.75 5.678
2.75 5.678
};
\addplot [black]
table {%
3 5.678
3 5.678
};
\addplot [black]
table {%
3 5.678
3 5.678
};
\addplot [black]
table {%
2.875 5.678
3.125 5.678
};
\addplot [black]
table {%
2.875 5.678
3.125 5.678
};
\addplot [black]
table {%
3.75 5.431
4.25 5.431
4.25 5.6635
3.75 5.6635
3.75 5.431
};
\addplot [black]
table {%
4 5.431
4 5.355
};
\addplot [black]
table {%
4 5.6635
4 5.92
};
\addplot [black]
table {%
3.875 5.355
4.125 5.355
};
\addplot [black]
table {%
3.875 5.92
4.125 5.92
};
\addplot [black]
table {%
4.75 5.29018330574036
5.25 5.29018330574036
5.25 5.33972787857056
4.75 5.33972787857056
4.75 5.29018330574036
};
\addplot [black]
table {%
5 5.29018330574036
5 5.21857261657715
};
\addplot [black]
table {%
5 5.33972787857056
5 5.39882755279541
};
\addplot [black]
table {%
4.875 5.21857261657715
5.125 5.21857261657715
};
\addplot [black]
table {%
4.875 5.39882755279541
5.125 5.39882755279541
};
\path [draw=red, dash pattern=on 1pt off 1.65pt]
(axis cs:0.5,4.798)
--(axis cs:5.5,4.798);

\addplot [red]
table {%
0.75 6.14125
1.25 6.14125
};
\addplot [red]
table {%
1.75 5.772
2.25 5.772
};
\addplot [red]
table {%
2.75 5.678
3.25 5.678
};
\addplot [red]
table {%
3.75 5.528
4.25 5.528
};
\addplot [red]
table {%
4.75 5.3097939491272
5.25 5.3097939491272
};
\end{axis}

\end{tikzpicture}


==> Sections/old_abstract.tex <==
Flying a quadrotor through a series of waypoints in minimum time is very challenging due to complex dynamic effects and disturbances. These effects are very pronounced as the robot flies at the limits of its performance envelope.
%
%These effects are specially pronounced when flying at the absolute limits of the platform.
%
Recently, Model Predictive Contouring Control (MPCC) has arisen as the state-of-the-art approach for model-based minimum-time flight.
%
MPCC maximizes the progress along a nominal path directly within the optimization problem at runtime, achieving unprecedented results.
%
% By maximizing the progress along a nominal path directly within the optimization problem, MPCC optimally selects the future states of the platform at runtime, achieving astonishing results. 
%
% Instead of relying on a pre-computed, time-optimal, dynamically feasible path that takes hours to generate \cite{foehn2021CPC}, it directly maximizes the progress along a nominal path inside the optimization problem, at every control iteration.
%
% This has been shown to allow for faster laptimes, since the approach is constantly taking into account the current state of the platform to allocate in time the immediate next states in the horizon.
%
%
%
%
% The current state-of-the-art model-based approach is the receding horizon approach called Model Predictive Contouring Control (MPCC).
%
% By taking into account the full quadrotor model it 
%
%
% MPCC has achieved astonishing results in the task of flying in minimum time through a set of waypoints.
%
However, finding the optimal set of tuning parameters for MPCC is challenging because (i) the full quadrotor dynamics are non-linear, (ii) the cost function is highly non-convex, and (iii) of the high dimensionality of the hyperparameter space.
% linearly grows with the number of waypoints to be passed.
%
In fact, it can take days for a human expert to manually tune said MPCC controller for minimum-time flight. 
%
% \davide{You have to  mention the sota for this task: AutoTune}
%
% Recent advances in model-based control have led to a very successful
% intro
% Cost function design is one of the most recurrent challenges today in robotics, for both model-based and learning-based approaches.
% Is it possible to combine the flexibility that Reinforcement Learning offers in terms of reward shaping with the interpretability and domain knowledge that is inherently encoded in a model-based architecture?
%
% Model-free Reinforcement Learning approaches have shown to perform extremely well in a variety of tasks, but they often suffer from a lack of interpretability and from high sample complexity.
%
% On the other hand, model-based methods can exploit domain knowledge to be more sample efficient, but often require a tuning step manually done by a human expert with domain knowledge.
%
In this paper, we apply Policy Search to automatically tune an MPCC to fly a quadcopter for the task of minimum-time flight through a series of waypoints.
\yunlong{I would be very careful when using the word RL. The method that we are using is called weighted maximum likelihood. Essentially, this is not RL, but belongs to probabilistic inference in general machine learning. } \davide{I removed RL, please check.}

%
%We apply model-free Reinforcement Learning Policy Search in order to search for optimal set of hyperparameters. 
%
%Because it uses a model-based controller, the approach incorporates and benefits from knowledge of the model. 
%
The data efficiency provided by the use of a model-based approach allows us to directly train in a high-fidelity simulator, which in turn makes our approach able to transfer zero-shot to the real-world.
%
We compare our approach to both both hand-tuning by human expert and the state-of-the-art, auto-tuning baseline and show that we outperform it by X\%. \davide{I added hand-tuning baseline too.}
%
% We showcase our approach by tuning the MPCC controller in the task of drone racing.
% %
% The results are better and achieve faster laptimes than when human experts manually tune the controller.
We validate our approach in the real world, where we show that our  method outperforms both the previous manually tuned controller and world-class human pilots by achieving  speeds  of  up  to  75 km/h.\davide{I dont recall your MPCC to outperform Vanover and Bitmatta, am I missing something?}



==> Sections/old_intro.tex <==



% Model Predictive Contouring Control \cite{}
When it comes to speed, quadrotors are among the most dynamic and agile flying devices ever built \cite{spectrum2020acrobatics}. 
%
Flying these machines at the limit of their actuation is extremely challenging and has recently gained large interest in the robotics community in the context of drone racing \cite{foehn2021CPC, feigaoracing, Foehn20rss}.

\yunlong{The following paragraph talks about drone racing. IMO, maybe not necessary. we can focus on generally agile flight.
The paper is about tunning a controller for agile flight. }
The goal of drone racing is to fly a quadrotor through a series of gates in a given order in minimum time. 
%
This problem is also referred to as time-optimal waypoint flight, or simply time-optimal flight. 
%
This task requires control algorithms that operate the vehicle at the limit of its performance envelope: high speed, high accelerations, high accuracy, high uncertainty, low reaction time, and an extremely low tolerance for mistakes.
%
World-class human pilots take years of experience to develop the dexterity, reflexes, and sensorimotor skills needed to win at a drone race.
%
Therefore, addressing this problem allows unlocking the full potential of the vehicle, ultimately pushing the frontiers of current and emerging real-world applications.
%
% Both model-based and model-free approaches have been used to solve the task of steering these type of platforms through complex environments. \angel{cite robert paper, cite CPC again, cite MPCC}
%

Recently, Model Predictive Contouring Control (MPCC)  has arisen as the state-of-the-art approach for model-based time-optimal flight~\cite{mpcc_tro, mpcc_replanning}.
%
In contrast to classical planning and control pipelines (which rely on a pre-computed, time-optimal, dynamically feasible path that takes hours to generate \cite{foehn2021CPC}), MPCC directly maximizes the progress along a nominal path inside the optimization problem, at every control iteration.
%
MPCC uses the current state of the platform to find the optimal time allocation of the immediate next states in the prediction horizon. 
%
This has been shown to lead to faster lap times than the state-of-the-art in classical planning and control pipelines: a standard MPC controller tracking a time-optimal trajectory~\cite{foehn2021CPC, mpcc_tro}.
%

% \begin{figure}[t!]
%   \centering
%   \includegraphics[width=0.5\textwidth]{Figures/BLOCK-RL.pdf}
%   \caption{An overview of the proposed \textit{policy-search-for-model-predictive-control framework}. TODO: [add image to guassian, modify background, add simulation text] }
%  \label{fig: method_overview}
% \end{figure}

However, finding the right tuning parameters of an MPCC controller for time-optimal flight is extremely challenging because a) the full quadrotor dynamics are non-linear; b) the cost function of the controller is highly complex and non-convex; and c) the dimensionality of the hyperparameter space is high and grows linearly with the amount of gates to be passed.
%
Because of these reasons, it takes a human expert days or even weeks to find an optimal set of tuning parameters for a specific track layout. A manual choice is most likely sub-optimal.
%

There are different existing approaches for automatic controller tuning. 
%
% The traditional approach for automatic tuning known as the MIT rule \cite{MITrule}, was developed inside the frame of adaptive control.
% %
% It requires that the metric to be optimized is expressed as a quadratic function of the controller parameters, and then optimizes the controller with gradient-based optimization \cite{grimble1984implicit, aastrom1993automatic, mohd2015intelligent}.
% %
% However, expressing the long term measure (in our case the laptime and gate passing metrics) as a function of the tuning parameters is impractical and generally intractable.
% %
% Instead of analytically computing it, another line of work proposes to iteratively estimate the optimization function, and use the estimate to find optimal parameters \cite{menner2020maximum, berkenkamp2016safe, marco2016automatic}.
% %
% However, these methods make over-simplifying assumptions on the objective function, e.g. convexity or relative Gaussianity between observations. Such assumptions are generally not suited for controller tuning to high-speed flight, where the function is highly non-convex.
%
Specifically in the context of racing, one approach that has shown promising results in the domain of car racing is \cite{BOZeilinger}, where they use Bayesian Optimization in order to jointly optimize the parameters of the dynamic model and tuning parameters of an MPCC architecture.
%
Another related approach that deals directly with receding horizon controller tuning for agile flight is AutoTune~\cite{autotune}, and has its roots in statistical learning. 
%
AutoTune can cope with sparse metrics such as lap times or gate collisions directly. 
%
It samples the metric function using Metropolis-Hasting, an efficient version of Monte Carlo sampling that is non-gradient based.
%
While AutoTune has shown to outperform existing methods, it has difficulties when dealing with controllers where the dimensionality of the parameter space increases.
%
As a matter of fact, both these related works have only dealt with a relatively small dimensionality in the parameter space (less than 10 parameters).
%


Recently, model-free Reinforcement Learning (RL) approaches have demonstrated impressive results in controlling very complex systems \cite{degrave2022magnetic, marcohutter2020}. In particular, Policy Search methods have successfully been used for tuning a Model Predictive Controller (MPC) to perform agile flight with in very complex environments \cite{yunlong_policy}. This work exploits the advantages of RL to learn complex policies using experienced data and applies them to achieve adaptive and optimal control performance in the task of agilely flying through fast-moving gates.


%
% On the other hand, model-free reinforcement learning (RL) approaches have demonstrated impressive results in very complex tasks \cite{marcohutter2020}.
% \angel{work on this connecting part more}

% %
% One of the key advantages of model-free approaches is that they can handle very sparse objectives that can be directly written as a reward function.
%
%However, model-based optimal control approaches need to first encode the objective such that the optimization problem to be solved is well defined, mostly through a set of high level hyperparameters that need to be tuned by hand.
%


% In this paper, the aim is to combine the high flexibility in task definition via a reward function that model-free Reinforcement Learning (RL) approaches benefits from. 
%
% One of the key advantages of RL is that it can handle very sparse objectives, encoded in the form of a reward function, whereas for optimal control methods, the approach itself needs to be engineered and hand-crafted given a high level task.
%
%
% In order to do this, we narrow the problem to a specific task: tuning a model-based controller for drone racing.
%
% We use autonomous drone racing as the domain for examining our hypotheses.
% % 
% The task is to fly a quadrotor through a sequence of gates in minimum time.
% 
% Drone racing serves as the perfect benchmark to advance the state-of-the-art in the field of robotics because it covers the entire envelope of challenges that the robotics community needs to solve.
%
%

% In this paper, we address the following research questions: can we train an RL agent in simulation that can find a combination of MPCC hyperparameters that result in better performance than the best hand-tuned controller? Does this tuning transfer directly to the real-world?
%
In this paper, we propose the use of Policy Search \cite{yunlong_policy} for searching the space of hyperparameters of an MPCC controller.
% \angel{describe how good policy search solves the task of looking for hyperparameters for the task of agilely flying through moving gate}
% The state-of-the-art in model-based control to solve the task of drone racing is Model Predictive Contouring Control (MPCC).
%
% MPCC has been architectured and manually tuned to solve the task of drone racing.
%
% By maximizing progress directly at optimization time, it has shown to be able to outrace expert human pilots.
%
% However, one of its disadvantages is the tremendous effort that needs to be put in order to manually find a combination of high level parameters that leads to good performance, a choice that is very likely to be suboptimal.
% \subsection{Why is the problem hard, what makes it challenging?}
%
%Additionally, to automatically find the best combination of tuning parameters for our controller given a high-level reward, we need to find (or approximate) the gradient of our controller with respect to its tuning parameters.
%
%The main challenge is that in order to approximate this gradient, we need to solve several times a complex non linear optimization problem. 
%
%Every sample of the reward function means an entire experiment where the optimizer is sampled several thousand times.
%
% \subsection{How far has existing work come? What is the next frontier?}
%
% \subsection{Why hasn't the problem been solved, what is the stumbling block?}
% \subsection{What does our paper contribute}
%
In contrast to end-to-end learning, where the agent needs to learn everything from data, having an optimal controller in the loop leverages the use of a model by the optimizer, which allows a sample efficiency that permits training in a very complex, hyperrealistic simulation \cite{bauersfeld2021neurobem}. 
%
We show that the controller has the ability to transfer zero-shot to the real world by flying extremely agile maneuvers through a set of two different tracks designed by one of the best professional drone pilots in the world.


% \subsection{What is the key idea? What is the magic trick?}
% \subsection{What do the expriments say?}


\subsection*{Contributions}
The contributions of this paper are threefold: a) we are able to automatically find the optimal hyperparameters for an MPCC controller which ultimately results in the best ever laptimes achieved with this approach, outperforming those found by an expert human after weeks of parameter tuning in the real-world; b) by leveraging the inherent data efficiency of using a model-based approach in the loop, we are able for the first time to train in a hyperrealistic simulator; and c) we demonstrate the ability to transfer the results obtained in simulation zero shot to the real world by flying through two different tracks at speeds up to 75 km/h.



==> Tables/baseline_gate_error.tex <==
{
\renewcommand{\arraystretch}{1.5}
\begin{table*}[!htp]
    \centering
    \setlength{\tabcolsep}{3pt}
    \caption{A baseline comparison of different methods for drone racing.}
    \label{tab:results_overview}
    \begin{tabular}{c c cc cc cc cc cc}
        \toprule
        \multirow{2}{*}{\begin{minipage}{5mm} Race\\Track\end{minipage}} & \multirow{2}{*}{\begin{minipage}{15mm}Simulation\\Environment\end{minipage}} 
        &  \multicolumn{2}{c}{Time Optimal~\cite{foehn2021CPC}}
        &  \multicolumn{2}{c}{MPC+CPC~\cite{foehn2021CPC}} 
        &  \multicolumn{2}{c}{MPCC+CPC~\cite{romero2021model}} 
        &  \multicolumn{2}{c}{Black Box~\cite{ryou2021multi} }
        &  \multicolumn{2}{c}{\textbf{RL (Ours)}} \\
        \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12}
        & & Lap Time & Passing Dist. & Lap Time & Passing Dist. & Lap Time  & Passing Dist. & Lap Time  & Passing Dist. & Lap Time  & Passing Dist.  \\
        \hline
        \multirow{2}{*}{Straight} 
        & Simple & \multirow{2}{*}{0.612}  & \multirow{2}{*}{-}  & 0.66 &  0.24 $\pm$ 0.14 &  0.70 & 0.074 $\pm$ 0.03  & x&x & 0.66 & 0.05 $\pm$ 0.03\\
        & BEM  & &   & 0.69 & 0.18 $\pm$ 0.14  & 0.74 & 0.13 $\pm$ 0.09  & x&x & 0.70 & 0.02 $\pm$ 0.01 \\
        \hline
        \multirow{2}{*}{Vertical} 
        & Simple & \multirow{2}{*}{0.764}  & \multirow{2}{*}{-}  & 1.53 & 0.00 $\pm$ 0.00  & 1.64 & 0.00 $\pm$ 0.00  & x&x & 0.88 & 0.09 $\pm$ 0.13\\
        & BEM  & &   & 1.44 & 0.00 $\pm$ 0.00 & 1.52 & 0.00 $\pm$ 0.00 & x&x & 0.92 & 0.09 $\pm$ 0.03 \\
        \hline
        \multirow{2}{*}{Marvin} 
        & Simple & \multirow{2}{*}{5.989}  & \multirow{2}{*}{-}  & x & x $\pm$ x   & x&x   & x&x  & 7.05 & 0.21 $\pm$ 0.13  \\
        & BEM  & & & x & x $\pm$ x & x & x  & x&x & 7.36 & 0.39 $\pm$ 0.16 \\
        \hline
        \multirow{2}{*}{SplitS}  
        & Simple & \multirow{2}{*}{4.798}  & \multirow{2}{*}{-}   & x&x &  5.150 & 0.232  $\pm$ 0.174  & x&x  & 5.00 & 0.16 $\pm$ 0.08  \\
        & BEM  & &  & x&x & 5.234 & 0.361 $\pm$ 0.134 & x&x  & 5.06 & 0.39 $\pm$ 0.24 \\
        \bottomrule
    \end{tabular}
\end{table*}
}



==> Tables/baselines.tex <==
{
\renewcommand{\arraystretch}{1.5}
\begin{table*}[!htp]
    \centering
    \setlength{\tabcolsep}{3pt}
    \caption{A baseline comparison of different methods for drone racing.}
    \label{tab:results_overview}
    \begin{tabular}{c c c c c c}
        \toprule
        \multirow{2}{*}{\begin{minipage}{5mm} Race\\Track\end{minipage}} & \multirow{2}{*}{\begin{minipage}{15mm}Simulation\\Environment\end{minipage}}
        & {Time Optimal~\cite{foehn2021CPC}}
        & {MPC+CPC~\cite{foehn2021CPC}} 
        & {MPCC+CPC~\cite{romero2021model}} 
        & {\textbf{RL (Ours)}} \\
        % & \cmidrule(lr){3} \cmidrule(lr){4} \cmidrule(lr){5} \cmidrule(lr){6} \\
        && Lap Time ($s$) & Lap Time ($s$) & Lap Time ($s$) & Lap Time ($s$)  \\
        \hline
        \multirow{2}{*}{Straight} 
        & Simple & 0.612  & 0.62 &  0.70 & 0.66 \\
        & BEM  & - & 0.66 & 0.74 & 0.70 \\
        \hline
        \multirow{2}{*}{Vertical} 
        & Simple & 0.758  & 1.69 & 1.64 & 0.88 \\
        & BEM  & -  & 1.57 & 1.52 & 0.92 \\
        \hline
        \multirow{2}{*}{Race Track 1}  
        & Simple & 4.836  & 5.38 &  5.150 & 5.00  \\
        & BEM  & - & 5.37 & 5.234  & 5.06  \\
        \hline
        \multirow{2}{*}{Race Track 2} 
        & Simple & 6.796 & 7.58* &  -  & 7.05   \\
        & BEM  & - & 7.58* & - &  7.36  \\
        \bottomrule
    \end{tabular}
\end{table*}
}



==> Tables/quad_config.tex <==
\begin{table}[htp]
    \centering
    \setlength{\tabcolsep}{3pt}
    \caption{Quadrotor Configurations}
    \label{tab:quads}
    \begin{tabular}{cl||c}
        \toprule
        \rowcolor{Gray}
        \multicolumn{2}{c||}{Parameter} & Nominal Value\\
        \midrule
        $m$& $[\si{\kilo\gram}]$ & $0.752$ \\
        $\boldsymbol{I}_v$& $[\si{\gram\meter^2}]$ & $\mathrm{diag}(2.5, 2.1, 4.3)$  \\
        $\left(u_\mathrm{min}, u_\mathrm{max}\right)$& $[\si{\newton}]$ & $\left(0, 8.5\right)$  \\
        $c_q$& $[\si{Nm^2}]$ & $2.37e^{-8}$ \\
        $c_t$& $[\si{N^2}]$ & $1.51e^{-6}$  \\
        $\left(k_{d,x},~k_{d,y},~k_{d,z}\right)$& $[\si{kg/s}]$ & $\left(0.26,~0.28,~0.42\right)$ \\
        $k_{h}$& $[\si{kg/m}]$ & $0.01$ \\
        $\delta_{t}$& $[\si{ms}]$ & $40 \sim 80$  \\
        \bottomrule
    \end{tabular}
\end{table}

==> Tables/racing_baselines.tex <==
{
\renewcommand{\arraystretch}{1.5}
\begin{table}[!htp]
    \centering
    \setlength{\tabcolsep}{3pt}
    \caption{Baselines}
    \label{tab:results_overview}
    \begin{tabular}{c|c|c|c}
        \toprule
        \rowcolor{Gray}
        Method & Environment & Lap Time ($\si{s}$) & Gate Passing Errors (\si{m})  \\
        \hline
        \multirow{2}{*}{MPCC} 
        & Simple & 5.150 $\pm$ 0.014 & 0.232 $\pm$ 0.174     \\
        & BEM & 5.234 $\pm$ 0.022 & 0.361 $\pm$ 0.134    \\
        \hline
        \multirow{2}{*}{MPC} 
        & Simple & 6.120 $\pm$  0.000 & $\pm$     \\
        & BEM & 6.120 $\pm$ 0.000 & $\pm$    \\
        \hline
        \multirow{2}{*}{RL (Ours)} 
        & Simple & 5.184  $\pm$ 0.030  &  0.121 $\pm$ 0.058    \\
        & BEM & 5.216 $\pm$ 0.011  & 0.367 $\pm$ 0.201    \\
        % \hline
        % \multirow{2}{*}{TCN (Ours)} 
        % & Simple & 5.235 $\pm$ 0.009 &  0.094 $\pm$ 0.030     \\
        % & BEM & 5.242 $\pm$ 0.021 & 0.498 $\pm$ 0.233    \\
        % \hline
        % \multirow{2}{*}{RNN (Ours)} 
        % & Simple & 5.180 $\pm$ 0.014 & 0.111 $\pm$ 0.042    \\
        % & BEM & 5.250 $\pm$  0.015 & 0.451 $\pm$ 0.217    \\
        \bottomrule
    \end{tabular}
\end{table}
}



==> tikz/tikz_gaussian.tex <==
\newcommand\gauss[2]{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))} % Gauss function, parameters mu and sigma
\begin{tikzpicture}
\begin{axis}[axis x line=none, axis y line=none, axis x line shift=-0.06cm, axis line style = thick, xtick=\empty, ytick=\empty, every axis plot post/.append style={
    mark=none,domain=-2.5:2.5,samples=50,smooth, thick},
  xmin=-3,xmax=3,ymin=0,ymax=1.5,
  xlabel={}, ylabel={}, xlabel style={xshift=0.45cm, yshift=0.5cm}] % All plots: from -2:2, 50 samples, smooth, no marks
\draw[->, very thick] (axis cs: -2.0, 0.7) to [out = 0, in=180]
    coordinate[pos=0.0] (x0)
    coordinate[pos=0.2] (x1)
    coordinate[pos=0.4] (x2)
    coordinate[pos=0.6] (x3)
    coordinate[pos=0.8] (x4)
    coordinate[pos=1.0] (xend)
    (axis cs: 2.0, 0.3);
\fill[black] (x0) circle (2pt);
\fill[black] (x1) circle (2pt);
\fill[black] (x2) circle (2pt);
\fill[black] (x3) circle (2pt);
\fill[black] (x4) circle (2pt);

\node[text=black] at ([yshift=0.25cm]x0) {\tiny $\boldsymbol{k{=}0}$};
\node[text=black] at ([yshift=0.25cm]x1) {\tiny $\boldsymbol{k{=}1}$};
\node[text=black] at ([yshift=0.25cm]x2) {\tiny $\boldsymbol{k{=}2}$};

% \node[text=black] at ([yshift=0.4cm]xend) {$\boldsymbol{p^d_x(\theta_k)}$};
\node[text=black] at ([yshift=0.4cm]xend) {$\boldsymbol{p_x(k)}$};
\addplot [blue, opacity=0.5] {\gauss{0.35}{0.35} + 0.15};
% \node[text=blue] at (axis cs: 1.65, 1.1) {$\boldsymbol{q_c(p^d_x(\theta_k))}$};
\node[text=blue] at (axis cs: 1.65, 1.1) {$\boldsymbol{q_c(p_x(k))}$};
\draw [dashed, opacity=0.4] (x0) to ([yshift=-2.09cm]x0);
\draw [dashed, opacity=0.4] ([yshift=3.2cm]x3) to (x3);
% \node[text=black] at ([yshift=-0.4cm, xshift=0cm]x3) {\tiny $\boldsymbol{p^d_{x,g}(\theta_j)}$};

\fill[blue] ([yshift=-2.09cm]x0) circle (2pt);
\node[text=blue] at ([yshift=-1.9cm, xshift=-0.5cm]x0) {\footnotesize $\boldsymbol{q_{nom}}$};

\draw [dashed, opacity=0.4] (x1) to ([yshift=-1.92cm]x1);
\fill[blue] ([yshift=-1.92cm]x1) circle (2pt);

\draw [dashed, opacity=0.4] (x2) to ([yshift=-1.0cm]x2);
\fill[blue] ([yshift=-1.0cm]x2) circle (2pt);

\fill[blue] ([yshift=3.18cm]x3) circle (2pt);
\node[text=blue] at ([yshift=3.25cm, xshift=-0.5cm]x3) {\footnotesize $\boldsymbol{q_{wp}}$};

\draw [dashed, opacity=0.4] (x4) to ([yshift=-0.3cm]x4);
\fill[blue] ([yshift=-0.3cm]x4) circle (2pt);

\end{axis}
\end{tikzpicture}

